The geometry of multi-curve interest rate models

We study the problems of consistency and of the existence of finite-dimensional realizations for multi-curve interest rate models of Heath-Jarrow-Morton type, generalizing the geometric approach developed by T. Bj\"ork and co-authors in the classical single-curve setting. We characterize when a multi-curve interest rate model is consistent with a given parameterized family of forward curves and spreads and when a model can be realized by a finite-dimensional state process. We illustrate the general theory in a number of model classes and examples, providing explicit constructions of finite-dimensional realizations. Based on these theoretical results, we perform the calibration of a three-curve Hull-White model to market data and analyse the stability of the estimated parameters.

==> rm_09_2021_4m/OIS_bond_cubic_spline_IRS_rate_cubic_spline/attempt_1_error_table <==
\begin{tabular}{llll}
\toprule
{} &                  OIS &                      3M &                     6M \\
\midrule
yields &  0.07311786903582018 &     0.05698016359637451 &    0.05261442646646061 \\
spread &                    - &  2.6942328517402667e-07 &  4.874427004790017e-07 \\
\bottomrule
\end{tabular}


==> rm_09_2021_4m/OIS_bond_linear_IRS_rate_linear/attempt_1_error_table <==
\begin{tabular}{llll}
\toprule
{} &                   OIS &                     3M &                     6M \\
\midrule
yields &  0.019166664182416332 &   0.017050071549714406 &   0.023849750321755046 \\
spread &                     - &  6.929291244895871e-07 &  8.491171956112916e-07 \\
\bottomrule
\end{tabular}

